Chemical and stellar properties of early-type dwarf galaxies around the Milky Way

Early-type dwarfs (ETDs) are the end points of the evolution of low-mass galaxies whose gas supply has been extinguished. The cessation of star-formation lays bare the ancient stellar populations. A wealth of information is stored in the colours, magnitudes, metallicities and abundances of resolved stars of the dwarf spheroidal and ultra-faint galaxies around the Milky Way, allowing their chemistry and stellar populations to be studied in great detail. Here, we summarize our current understanding, which has advanced rapidly over the last decade thanks to the flourishing of large-scale astrometric, photometric and spectroscopic surveys. We emphasise that the primeval stellar populations in the ETDs provide a unique laboratory to study the physical conditions on small scales at epochs beyond z=2. We highlight the observed diversity of star-formation and chemical enrichment histories in nearby dwarfs. These data can not yet be fully deciphered to reveal the key processes in the dwarf evolution but the first successful attempts have been made to pin down the sites of heavy element production.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


